Adaptive Optimization Algorithms for Machine Learning

Machine learning assumes a pivotal role in our data-driven world. The increasing scale of models and datasets necessitates quick and reliable algorithms for model training. This dissertation investigates adaptivity in machine learning optimizers. The ensuing chapters are dedicated to various facets of adaptivity, including: 1. personalization and user-specific models via personalized loss, 2. provable post-training model adaptations via meta-learning, 3. learning unknown hyperparameters in real time via hyperparameter variance reduction, 4. fast O(1/k^2) global convergence of second-order methods via stepsized Newton method regardless of the initialization and choice basis, 5. fast and scalable second-order methods via low-dimensional updates. This thesis contributes novel insights, introduces new algorithms with improved convergence guarantees, and improves analyses of popular practical algorithms.

==> parts/papers/adaptive/sections/abstract.tex <==
Recent advances in the theoretical understanding of SGD \cite{SGD_general_analysis} led to a formula for the optimal   batch size  minimizing the number of effective data passes, i.e., the number of iterations times the   batch size. However, this formula is of no practical value as it depends on the knowledge of the variance of the stochastic gradients evaluated at the optimum.  In this paper we design a practical SGD method capable of learning the optimal   batch size adaptively throughout its iterations for strongly convex and smooth functions. Our method does this provably, and in our experiments with synthetic and real data robustly exhibits nearly optimal behaviour; that is, it works as if the optimal   batch size was known a-priori. Further,  we generalize our method to several new   batch strategies not considered in the literature before, including a sampling suitable for distributed implementations.


==> parts/papers/adaptive/sections/conclusion.tex <==
\section{Conclusion}

In this paper, We proposed a robust algorithm, which adaptively selects   batch sizes throughout training, that consistently performs almost as if we used SGD with optimal   batch size and theoretically grounded its convergence. Besides, we introduced generalized sampling strategies that are suitable for distributed optimization. We derived formulas for computing optimal   batch size, and empirically showed its precision.
The performance of our algorithm does not depend on the complexity of these formulas even when their computation required passing through the whole dataset. we employ an effective technique to efficiently utilize memory usage and avoid seeing non-sampled data-points.
The proposed algorithm can be viewed as an enhancement on SGD that is orthogonal to many other approaches (e.g., variance reduction). Thus, it might be possible to combine them in future work.


==> parts/papers/adaptive/sections/experiments.tex <==
\section{Experiments} \label{sec:experiments}

\begin{figure*}[t]
\begin{center}
\centerline{
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/mushrooms/Logistic_nice_mushrooms_1.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/mushrooms/Logistic_nice_mushrooms_2.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/mushrooms/Logistic_nice_mushrooms_3.png}
\includegraphics[width=0.25\textwidth, height = 66 pt]{figures/Complexity/Logistic_nice_mushrooms_1.png}
}
\centerline{
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/a1a/Logistic_ind_a1a_1.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/a1a/Logistic_ind_a1a_2.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/a1a/Logistic_ind_a1a_3.png}
\includegraphics[width=0.25\textwidth, height = 66 pt]{figures/Complexity/Logistic_nice_a1a_1.png}
}
\caption{\textbf{Convergence of logistic regression} using $\tau-$partition nice sampling on \emph{mushroom} dataset (first row) and $\tau-$partition independent sampling on \emph{a1a} dataset (second row). In first three columns, training set is distributed among $1$, $2$ and $3$ partitions, respectively. Figures in the fourth column show how many epochs does the SGD need to converge for all   batch sizes (single partition dataset).
}
\label{fig:logistic_nice}
\end{center}
\vspace{-0.75cm}
\end{figure*}

In this section, we compare our algorithm to fixed   batch size SGD in terms of the number of epochs needed to reach a pre-specified neighborhood $\epsilon/10$. In the following results, we capture the convergence rate by recording the relative error $(\nicefrac{\norm{x^k - x^*}^2}{\norm{x^0 - x^*}^2})$ where $x^0$ is drawn from a standard normal distribution $\mathcal{N}(0, \mathbf{I})$. We also report the number of training examples $n$, the dimension of the machine learning model $d$, regularization factor $\lambda$, and the target neighborhood $\epsilon$ above each figure.
We consider the problem of regularized ridge regression where each $f_i$ is strongly convex and L-smooth, and $x^*$ can be known a-priori and the classification problem through regularized logistic regression where the optimal model is attained by running gradient descent for a long time. Both problem can be mathematically formulated in the form $\min_{x \in \mathbb R^d} f(x)$ where
% The $l_2$ regularized logistic regression. 
% The $l_2$ regularized ridge regression can be formulated as:
\[ f_{\text{ridge}}(x) = \tfrac{1}{2n}\sum \limits_{i=1}^n \norm{a_i^T x - b_i}^2_2 + \tfrac{\lambda}{2}\norm{x}^2_2, \quad f_{\text{logistic}}(x) = \tfrac{1}{2n}\sum \limits_{i=1}^n\log\left(1+\exp \left(b_i a_i^T x\right)\right) + \tfrac{\lambda}{2}\norm{x}^2_2\]
% Also, we consider the classification problem through regularized logistic regression where the optimal model is attained by running gradient descent for a long time. 
% The $l_2$ regularized logistic regression can be formulated as:
% $$\min_{x \in \mathbb R^d} f(x) = \tfrac{1}{2n}\sum \limits_{i=1}^n\log\left(1+\exp \left(b_i a_i^T x\right)\right) + \tfrac{\lambda}{2}\norm{x}^2_2,$$
where $(a_i, b_i) \sim \mathcal{D}$ are pairs of data examples from the training set, and $\lambda > 0$ is the regularization coefficient.
For each of the considered problems, we performed experiments on at least two real datasets from LIBSVM \cite{libsvm}. We tested our algorithm on ridge regression on \emph{bodyfat} and \emph{mg} datasets in Figure \ref{fig:ridge_nice}. Results on logistic regression on \emph{mushrooms} and \emph{a1a} datasets are in Figure \ref{fig:logistic_nice}. 
For each of these datasets, we considered $\tau-$partition independent and $\tau-$partition nice sampling with distributing the training set into one, two, and three partitions.  
Moreover, we take the previous experiments one step further by running a comparison of various fixed   batch size SGD, as well as our adaptive method with a single partition (last column of Figures \ref{fig:ridge_nice} and \ref{fig:logistic_nice}).
We plot the total iteration complexity for each   batch size, and highlight optimal   batch size obtained from our theoretical analysis, and how many epochs our adaptive algorithm needs to converge. This plot can be viewed as a summary of grid-search for optimal   batch size (throughout all possible fixed   batch sizes). 
% In Table \ref{tb:the_only_table}, we record the interval of   batch sizes that outperform our algorithm and the percentage of   batch sizes that we outperform. Also, we compute the maximum speedup of our algorithm compared to fixed   batch size SGD ($\max_{\tau}\frac{T(\tau)}{T_\text{adaptive}}$, where $T_\text{adaptive}$ is the total complexity of our algorithm).

Despite the fact that the optimal   batch size is nontrivial and varies significantly with the model, dataset, sampling strategy, and number of partitions, our algorithm demonstrated consistent performance overall. In some cases, it was even able to cut down the number of epochs needed to reach the desired error to a factor of six. We refer the interested reader to the appendix for more experiments, on other datasets, different sampling strategies, and a different number of partitions.


The produced figures of our grid-search perfectly capture the tightness of our theoretical analysis. In particular, the total iteration complexity decreases linearly up to a neighborhood of $\tau^*$ and then increases linearly, as discussed in section \ref{sec:analysis}. In addition, Theorem \ref{le:tau_star} always captures the empirical minimum of $T(\tau)$ up to a negligible error. 
Moreover, these figures show how close $T_\text{adaptive}$ is to the total iteration complexity using optimal   batch size $T(\tau^*)$.
In terms of practical performance, our algorithm can be better than running SGD with $90\%$ of all possible fixed   batch sizes. This demonstrates that running the proposed algorithm is equivalent to ``guessing'' the optimal   batch size a-priori and hitting the interval of size $10\%$ around the optimal   batch size.

Finally, in terms of running time, the proposed algorithm is slightly more expensive than running vanilla SGD, since we estimate few parameters at each iteration. However, all of these estimates can be done through direct substitution to their formulas, which can be done cheaply. For example, on the \emph{bodyfat} experiment, the proposed algorithm requires $0.2322$ ms per epoch, while running SGD with the optimal   batch size requires $0.2298$ ms.

% \begin{table}
% \centering
% \caption{\textbf{Performance of Algorithm \ref{alg:sgd_dyn_general}} compared to fixed   batch size SGD. We report the interval where it outperforms our algorithm, the percentage where we prevail, and the maximum achieved speedup.}
% \vspace{0.3cm}
% \centering
% \begin{tabular}{c|ccc}
% \toprule
% Dataset    & Interval & Percentage & Speedup  \\
% \midrule

% \emph{bodyfat}          & $(48,84)$ & $85.3\%$ &$\sim \textit{x}3.5 $\\\hline
% \emph{mg}          & $(208, 454)$ & $82.5\%$ &$\sim \textit{x}3 $\\\hline
% \emph{mushrooms}          & $(2573, 3371)$ & $90.2\%$ &$\sim \textit{x}2 $\\\hline
% \emph{a1a}         & $(959, 1152)$ &$87.9\%$ & $ \sim \textit{x}2.5$\\
% \toprule
% \end{tabular}
% \label{tb:the_only_table}
% \vspace{-0.5 cm}
% \end{table}


==> parts/papers/adaptive/sections/introduction.tex <==


\section{Introduction}

Stochastic Gradient Descent (SGD), in one disguise or another, is undoubtedly the backbone of modern systems for training supervised machine learning models~\cite{robbins1951stochastic, nemirovski2009robust, bottou2010large}. The method earns its popularity due to its superior performance on very large datasets where more traditional methods such as gradient descent (GD), relying on a pass through the entire training dataset before adjusting the model parameters, are simply too slow to be useful. In contrast, SGD in each iteration uses a small portion of the training data only (a  batch) to adjust the model parameters, and this process repeats until a model of suitable quality is found. 

In practice,  batch SGD is virtually always  applied to a ``finite-sum'' problem of the form
\begin{equation} \label{eq:ERM}
  \textstyle  x^* \eqdef \arg \min \limits_{x\in \R} \frac{1}{n} \sum \limits_{i = 1}^n f_i(x),
\end{equation}
where $n$ is the number of training data and $f(x)=\frac{1}{n} \sum_{i = 1}^n f_i(x)$ represents the average loss, i.e.\ empirical risk, of model $x$ on the training dataset. With this formalism in place, a generic  batch SGD method performs iterations 
of the form
\begin{equation} \label{eq:SGD-MB}
\textstyle x^{k+1} = x^k - \gamma^k \sum \limits_{i\in S^k} v_i^k \nabla f_i(x^k),
\end{equation}
where $S^k \subseteq \{1,2,\dots,n\}$ is the  batch considered in iteration $k$ and $v_1^k,\dots,v_n^k$ are appropriately chosen scalars. Often in practice, and almost invariably in theory, the  batch $S^k$ is chosen at random according to some fixed probability law, and the scalars $v_i^k$ are chosen to ensure that $\textstyle g^k=\sum \limits_{i\in S^k} v_i^k \nabla f_i(x^k)$
% \begin{equation} \label{eq:g^k}
% \textstyle g^k=\sum \limits_{i\in S^k} v_i^k \nabla f_i(x^k)
% \end{equation}
is an unbiased estimator of the gradient $\nabla f(x^k)$. One standard choice is to fix a  batch size $\tau \in \{1,2,\dots,n\}$, and pick $S^k$ uniformly from all subsets of size $\tau$. Another option is to partition the training dataset into $n/\tau$ subsets of size $\tau$, and then in each iteration let $S^k$ to be one of these partitions, chosen with some probability, e.g., uniformly.

% \subsection{Accurate modelling of the second moment}
\textbf{Accurate modelling of the second moment}.
Despite the vast empirical evidence of the efficiency of  batch SGD \cite{minibatch}, and despite ample theoretical research in this area \cite{cotter2011better, li2014efficient, gazagnadou2019optimal, dont_decrease_step_size}, our understanding of this method is far from complete.  For instance, while it is intuitively clear that as the  batch size approaches $n$ the method should increasingly behave as the full batch GD method, the prevalent theory does not support this. The key reason for this, as explained by \cite{SGD_general_analysis} who consider the regime where all functions $f_i$ are smooth, and $f$ is (quasi) strongly convex, is inappropriate theoretical modelling of the second moment of the stochastic gradient $g^k$, which is not satisfied for stochastic gradients having the  batch structure. Indeed, a typical analysis of SGD assumes that there exists a constant $\sigma^2>0$ such that $\Exp{\norm{g^k}^2 \;|\ x^k} \leq \sigma^2$
% \begin{equation} \label{eq:b978dg9f}
% \Exp{\norm{g^k}^2 \;|\ x^k} \leq \sigma^2
% \end{equation}
holds throughout the iterations of SGD. However, this is not true for GD, seen as an extreme case of  batch SGD, which always sets $S^k=\{1,2,\dots,n\}$, and does not hold in general for any  batch size. Hence, analyses relying on this assumption are not only incorrect for  batch SGD~\cite{nguyen2018sgd}, but also make predictions which do not reflect empirical evidence. For instance, while practitioners have noticed that the choice $\tau>1$ leads to a faster method in practice even in a single processor regime, theory based on strong assumptions  does not predict this. Also, several works claim that the optimal batch size for SGD is one \cite{li2014efficient}.

Recently, \cite{SGD_general_analysis} studied the convergence of  batch SGD under a new type of assumption, called expected smoothness (ES). It is provably satisfied for stochastic gradients arising from  batching, and which is precise enough for all  batch sizes to lead to nontrivial predictions. Their assumption has the form $\Exp{\norm{g^k}^2 \;|\ x^k} \leq 2 A (f(x^k) - f(x^*)) + B$.
% \begin{equation}\label{eq:_ES}
%   \Exp{\norm{g^k}^2 \;|\ x^k} \leq 2 A (f(x^k) - f(x^*)) + B.  
% \end{equation}
When compared to the previous assumption, ES includes an additional term proportional to the functional suboptimality $f(x^k) - f(x^*)$.  In particular,  their analysis recovers the fast linear rate of GD in the extreme case when $\tau=n$ (in this case, ES holds with $B=0$ and $A=L$, where $L$ is the smoothness constant of $f$), and otherwise gives a linear rate to a neighborhood of the solution $x^*$ whose size depends on $B$. 

% \subsection{Search for the optimal  batch size}
\textbf{Search for the optimal  batch size}.
Of key importance to our work in this paper is a theoretical result in \cite{SGD_general_analysis} which characterizes the {\em optimal  batch size}. We will illustrate their result here on the example of the first of the two  batch schemes described in the introduction.  In particular, \cite{SGD_general_analysis} show that the {\em total  complexity} of  batch SGD to reach an $\epsilon$-neighborhood of the optimal solution $x^*$, i.e., the number of iterations multiplied by $\tau$,  is
\begin{equation} \label{eq:T} 
T(\tau) \eqdef  \max \left\{ \cK_1(\tau), \cK_2(\tau) \right\}
\end{equation}
where $\cK_1 \eqdef \tau(nL-L_{\max})+nL$ and $\cK_2\eqdef \tfrac{2(n-\tau)\Bar{h}(x^*)}{\mu\epsilon}$, $L$ is the smoothness constant of $f$, $L_{\max}$ is the maximum of the smoothness constants of the functions $f_i$, $\mu$ is the modulus of (quasi) strong convexity of $f$ and 
$\textstyle \Bar{h}(x) \eqdef \frac{1}{n}\sum \limits_{i=1}^n h_i(x),$
where $h_i(x) = \norm{\nabla f_i(x)}^2$. Since both $\cK_1$ and $\cK_2$ are both
linear functions in
$\tau$, the expression  $T(\tau)$ in \eqref{eq:T} can be analytically minimized in $\tau$, giving a formula for the optimal  batch size $\tau^*$ of SGD. 



\section{Contributions} \label{sec:contributions}
% \begin{wrapfigure}{r}{0.5\textwidth}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{birds}
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{center}
% \centerline{\includegraphics[width = 0.48\textwidth]{figures/tau_evolution/IterationComplexity.png}}
% \caption{\textbf{Number of epochs to converge} to $\epsilon$-neighborhood of the solution for different  batch sizes, tested on Logistic Regression using $\tau-$partition nice sampling on \emph{a1a} dataset. Our adaptive method outperforms SGD with $87.9\%$ of different fixed  batch sizes, achieving speedup up to $250\%$.}
% \label{fig:convergence_different_taus} 
% \end{center}
% % \vskip -0.4in
% \end{wrapfigure}

% \subsection{Motivation}
\textbf{Motivation}.
While the existence of a theoretically grounded formula for an optimal  batch size provides a marked step in the understanding of  batch SGD, the formula is not implementable in practice for several reasons. First, the quantity $\Bar{h}(x^*)$ is unknown as it depends on a-priori knowledge of the optimal solution $x^*$, which we are trying to find. One exception to this is the case of interpolated/overparameterized models characterized by the property that $\nabla f_i(x^*)=0$ for all $i$.

\begin{wrapfigure}{R}{0.5\textwidth}
\begin{center}
\centerline{\includegraphics[width = 0.45\textwidth]{figures/tau_evolution/IterationComplexity.png}}
\caption{\textbf{Number of epochs to converge} to $\epsilon$-neighborhood of the solution for different  batch sizes, tested on Logistic Regression using $\tau-$partition nice sampling on \emph{a1a} dataset. Our adaptive method outperforms SGD with $87.9\%$ of different fixed  batch sizes, achieving speedup up to $250\%$.}
\label{fig:convergence_different_taus} 
\end{center}
\vskip -0.3in
\end{wrapfigure}

However, in general, this property may not hold, and when it does, we may know this before we train the model. Second, the formula depends on the strong (quasi)-convexity parameter $\mu$, which also may not be known. Third, while the formula depends on the target accuracy $\epsilon$, in practice, we may not know what accuracy is most desirable in advance. 




Putting these parameter estimation issues aside, we may further ask: assuming these parameters are known, does the formula provide a good predictor for the behavior of  batch SGD? If it did not, it would be less useful, and perhaps inappropriate as a guide for setting the  batch size of SGD. \cite{SGD_general_analysis} showed through experiments with synthetic data that the optimal  batch size does well in cases when all these parameters are assumed to be known. However, they did not explore whether their formula \eqref{eq:T}  provides a good model for the {\em empirical} total complexity of  batch SGD across {\em all} values of $\tau$. The starting point of our research in this paper was investigating this question; the answer was rather surprising to us, as we illustrate in  Figure~\ref{fig:convergence_different_taus}. Our experiment shows that the theoretical predictions are astonishingly tight. The green V-shaped line reflects the empirical performance of SGD for various levels of  batch sizes, and correlates with the shape of the theoretical total complexity function $T(\tau)$. The orange vertical line depicts the theoretically optimal  batch size $\tau^*$, i.e., the solution to the problem $\min_{1 \leq \tau \leq n} T(\tau)$, and acts as a virtually perfect predictor of the optimal empirical performance. Encouraged by the above observation, we believe it is important to deliver the theoretically impractical formula for $\tau^*$ into the practical world, and this is the main focus of our paper. 
% \subsection{Summary of contributions}
In particular, we make the following contributions:

\textbf {Effective online learning of the optimal  batch size.} We make a step towards the development of a practical variant of optimal  batch SGD, aiming to learn the optimal  batch size $\tau^*$ on the fly. To the best of our knowledge, our method (Algorithm~\ref{alg:sgd_dyn_general}) is the first variant of SGD able to learn the optimal  batch.  The blue horizontal line in Figure~\ref{fig:convergence_different_taus} depicts the typical performance of our online method compared to  SGD with various fixed  batch sizes $\tau$. Our method can perform as if we had an almost perfect knowledge of $\tau^*$ available to us before the start of the method. Indeed, the blue line cuts across the green V-shaped curve in a small neighborhood of the optimal  batch size. 
% In this particular example, the speedup of our adaptive method compared to SGD with $\tau=1$ is approximately $250\%$. 


\textbf {Sampling strategies.} We do not limit our selves to the uniform sampling strategy we used for illustration purposes above and develop closed-form expressions for the optimal  batch size for other sampling techniques (Section~\ref{sec:analysis}). Our adaptive method works well for all of them.

\textbf {Convergence theory.} We prove that our adaptive method converges, and moreover learns the optimal  batch size (Section~\ref{sec:algo}; Theorem~\ref{th:convergence_our}).

\textbf {Practical robustness.} We show the algorithm's robustness by conducting extensive experiments using different sampling techniques and different machine learning models (Section~\ref{sec:experiments}).




\textbf{Related work}
% Many techniques have been designed in the literature to improve the performance of SGD in one way or another. 
A separate stream of research attempts to progressively reduce the variance of the stochastic gradient estimator aiming to obtain fast convergence to the solution, and not only to a neighborhood. SAG \cite{SAG}, SAGA \cite{SAGA}, SVRG \cite{SVRG},  L-SVRG \cite{L-SVRG-kovalev, L-SVRG-hoffman} and JacSketch \cite{jacsketch} are all examples of a large family of such variance reduced SGD methods. While we do not pursue this direction here, we point out that \cite{gazagnadou2019optimal} were able to specialize the JacSketch theory of \cite{jacsketch}  to derive expressions for the optimal  batch size of SAGA. A blend of this work and ours is perhaps possible and would lead to an adaptive method for learning the optimal  batch size of SAGA.

Another approach to boost the performance of SGD in practice is tuning its hyperparameters such as learning rate, and  batch size while training. In this context, a lot of work has been done in proposing various learning rate schedulers \cite{schumer1968adaptive, mathews1993stochastic,barzilai1988two,zeiler2012adadelta,tan2016barzilai,adaptive_step_size}. \cite{adaptive-mini-batch} showed that one can reduce the variance by increasing the  batch size without decreasing step-size (to maintain the constant signal to noise ratio). Besides, \cite{dont_decrease_step_size} demonstrated the effect of increasing the batch size instead of decreasing the learning rate in training a deep neural network. However, most of the strategies for hyper-parameter tuning are based on empirical results only. For example, \cite{you2017large,you2017scaling} show empirically the advantage of training on large  batch size, while \cite{masters2018revisiting} claim that it is preferable to train on small  batch sizes.


\section{SGD Overview}\label{sec:overview}
To proceed in developing the theory related to the optimal  batch size, we give a quick review of  batch SGD. To study such methods for virtually all (stationary) subsampling rules, we adopt the stochastic reformulation paradigm for finite-sum problems proposed in \cite{SGD_general_analysis}. For a given random vector $v \in \mathbb{R}^n$ sampled from a user defined distribution $\cD$ and satisfying $\mathbb{E}_{\mathcal{D}}[v_i] = 1$, the empirical risk in \eqref{eq:ERM} can be solved by taking the update step \eqref{eq:SGD-MB}.
% the main problem \eqref{eq:ERM} can be reformulated as
% $
% \min_{x\in \R}\mathbb{E}_{\mathcal{D}}\left[ f_v(x) = \tfrac{1}{n}\sum \limits_{i=1}^n v_i f_i(x)    \right].
% $
% This problem can be solved by applying SGD, i.e., in iteration $k$ we sample $v^k\sim \cD$ and take an SGD steps $x^{k+1} = x^k - \gamma^k \nabla f_{v_k}(x^k)$.  
Typically, the vector $v$ is defined by first choosing a random  batch $\cS^k\subseteq \{1,2,\dots,n\}$, and then defining $v_i^k  = 0$ for $i\notin \cS^k$, and choosing $v_i^k$ to an appropriate value for $i\notin \cS^k$ in order to make sure the stochastic gradient $\nabla f_{v^k}(x^k)$ is unbiased. 
% This leads to the the update rule \eqref{eq:SGD-MB} we mentioned in the introduction.
We will now briefly review four particular choices of the probability law governing the selection of the sets $\cS^k$ we consider in this paper.

\textbf{$\tau-$independent sampling} \cite{SGD_general_analysis}. In this sampling, each element is drawn independently with probability $p_i$ with $\sum_i p_i = \tau$ and $\mathbb{E}[|\mathcal{S}|] = \tau$. For each element $i$, we have $
\mathbbm P[v_i=\mathbbm 1_{i \in \mathcal S}]=p_i$. 

\textbf{$\tau-$nice sampling (without replacement)} \cite{SGD_general_analysis}. In this sampling, we choose subset of $\tau$ examples from the total of $n$ examples in the training set at each iteration. In this case, $P[|\mathcal{S}| = \tau] = 1$. For each subset $C \subseteq \{1,\dots, n \}$ of size $\tau$ , we have $\mathbb P[v_C=\mathbbm 1_{C \in \mathcal S}]=1/\binom n \tau$.

\textbf{$\tau-$partition nice sampling} In this sampling, we divide the training set into partitions $\mathcal C_j$ (of possibly different sizes $n_{\mathcal C_j}$), and each of them has at least a cardinality of $\tau$. At each iteration, one of the sets $\mathcal C_j$ is chosen with probability $q_{\mathcal C_j}$, and then $\tau-$nice sampling (without replacement) is applied on the chosen set. For each subset $C$ cardinality $\tau$ of partition $C_j$ cardinality $n_{C_j}$, we have $\mathbb P[v_C=\mathbbm 1_{C \in \mathcal S}]=q_j/\binom {n_{C_j}} \tau$. 

\textbf{$\tau-$partition independent sampling} Similar to $\tau-$partition nice sampling, we divide the training set into partitions $\mathcal C_j$, and each of them has at least a cardinality of $\tau$. At each iteration one of the sets $\mathcal C_j$ is chosen with probability $q_{\mathcal C_j}$, and then $\tau-$independent sampling is applied on the chosen set. For each element $i$ of partition $C_j$, we have $\mathbb P[v_i=\mathbbm 1_{C \in \mathcal S}]=q_jp_i$. 



Sampling using $\tau-$partition nice and $\tau-$partition independent sampling are the generalization of both $\tau-$nice (without replacement) and $\tau-$independent sampling respectively. Generalized samplings arise more often in practice whenever big datasets are distributed throughout different nodes. Consequently, it allows us to model a real situation where distributions of training examples throughout nodes might be very heterogeneous. These samplings are especially interesting to be analyzed because it can model distributed optimization where the data is partitioned across multiple servers within which the gradient of a batch is computed and communicated to a parameter server. 
The stochastic formulation naturally leads to the concept of expected smoothness, which can be defined as follows \cite{sega}

\begin{assumption}
\label{as:expected_smoothness}
A function $f$ is $\mathcal{L}-$smooth with respect to a datasets $\mathcal{D}$ if there exist $\mathcal{L} > 0$ such that
\begin{equation}\label{eq:exp_smoothn_cL}
\mathbb{E}_\mathcal{D}\left[\left\| \nabla f_v(x) - \nabla f_v(x^*) \right\|^2\right] \leq 2 \mathcal{L}(f(x) - f(x^*)). 
\end{equation}
\end{assumption}
The second assumption that the above formulation depends on is the finite gradient noise at the optimum which can be stated as follows \cite{SGD_general_analysis}
\begin{assumption}
\label{as:gradient_noise}
The gradient noise $\sg = \sg(x^*)$, where 
$    \sg(x) := \mathbb{E}_\mathcal{D}\left[\left\| \nabla f_v(x) \right\|^2  \right],
$
is finite.
\end{assumption}
% Assumptions \eqref{as:expected_smoothness} and \eqref{as:gradient_noise} can result in inequality \eqref{eq:_ES} by setting $A = 2\mathcal{L}$ and $B = 2\sigma$.
Based on the two assumptions, the update steps in \eqref{eq:SGD-MB} provide linear convergence up to a neighbourhood of the optimal point $x^*$. This convergence is described in the following theorem \cite{SGD_general_analysis}.
\begin{theorem}
\label{th:convergence_general}
Assume $f$ is $\mu-$strongly convex and Assumptions \ref{as:expected_smoothness}, \ref{as:gradient_noise} are satisfied. For any $\epsilon > 0$, if the learning rate $\gamma$ is set to be
\begin{equation} 
    \gamma = \tfrac 1 2 \min \left\{ \tfrac{1}{\mathcal{L}}, \tfrac{\epsilon \mu}{2\sg} \right\} \qquad  \text{and}\qquad k \geq \tfrac 2 {\mu} \max\left\{ \mathcal{L}, \tfrac{2\sg}{\epsilon \mu} \right\} \log\left( \tfrac{2 \|x^0 - x^*\|^2}{\epsilon} \right)\label{eq:iteration_complexity}
\end{equation}
% and 
% \begin{equation} \label{eq:iteration_complexity}
% k \geq \tfrac 2 {\mu} \max\left\{ \mathcal{L}, \tfrac{2\sg}{\epsilon \mu} \right\} \log\left( \tfrac{2 \|x^0 - x^*\|^2}{\epsilon} \right)
% \end{equation}
then $\mathbb{E} \left\| x^k - x^* \right\|^2  \leq \epsilon$.
\end{theorem}

% Inequality \eqref{eq:iteration_complexity} gives an upper bound for the number iterations required to guarantee convergence to $\epsilon$-neighborhood in the expectation. Note that in \eqref{eq:iteration_complexity} only parameters $\mathcal L$ and $\sg$ depend on $\tau$. In addition, in all the considered samplings, we find out that these parameters can have form $\frac{l(\tau)}{\tau}$ where $l$ is a piece-wise linear function, which is particularly crucial in our analysis. 



==> parts/papers/adaptive/sections/proposed_algorithm.tex <==
\section{Proposed Algorithm} \label{sec:algo}

% \begin{wrapfigure}{R}{0.5\textwidth}
% \begin{center}
% \centerline{\includegraphics[width = 0.45\textwidth]{figures/tau_evolution/IterationComplexity.png}}
% \caption{\textbf{Number of epochs to converge} to $\epsilon$-neighborhood of the solution for different   batch sizes, tested on Logistic Regression using $\tau-$partition nice sampling on \emph{a1a} dataset. Our adaptive method outperforms SGD with $87.9\%$ of different fixed   batch sizes, achieving speedup up to $250\%$.}
% \label{fig:convergence_different_taus} 
% \end{center}
% \vskip -0.3in
% \end{wrapfigure}

% \begin{wrapfigure}{R}{0.5\textwidth}
% \begin{minipage}{0.48\textwidth}
% \begin{algorithm}[H]
% \caption{SGD with Adaptive Batch size}
% \label{alg:sgd_dyn_general}
% \begin{algorithmic}
% \STATE \textbf{Input:} Smoothness constants $L$, $L_i$, strong convexity constant $\mu$, target neighborhood $\epsilon$, Sampling Strategy $S$, initial point $x^0$, variance cap $C \geq 0$
% \STATE \textbf{Initialize:} Set $k=0$
% \WHILE{not converged}
%     \STATE Set $\tau^k \leftarrow \tau(x^k)$ 
%     \STATE Set $\lk \leftarrow \mathcal L(\tau^k)$
%     \STATE Set $\sg^k \leftarrow \sg(x^k, \tau^k)$
%     \STATE Set $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min(C,2\sg^k)} \right\}$ 
%     \STATE Sample $v_k$ from $S$
%     \STATE Do SGD step: $x^{k+1} \leftarrow x^k - \gamma^k \nabla f_{v_k} (x^k)$
%     \STATE Update $k \leftarrow k+1$
% \ENDWHILE
% \STATE \textbf{Output:} $x^k$
% \end{algorithmic}
% \end{algorithm}
% \end{minipage}
% \end{wrapfigure}
% \begin{wrapfigure}{L}{0.48\textwidth}
% \begin{center}
% \centerline{
% \includegraphics[width=0.24\columnwidth]{figures/saga_experiments/mushrooms/Logistic_nice_Tau_mushrooms_1.png}
% \includegraphics[width=0.24\columnwidth,height=63.5pt]{figures/tau_evolution/logistic_nice_tau_a1a_1.png}
% }

% \centerline{
% \includegraphics[width=0.24\columnwidth]{figures/tau_evolution/ridge_nice_tau_bodyfat_1.png}
% \includegraphics[width=0.24\columnwidth]{figures/tau_evolution/ridge_ind_tau_mg_1.png}
% }
% \caption{\textbf{Behavior of $\tau-$adaptive throughout training epochs.} First row: logistic regression on \emph{mushroom} and \emph{a1a} datasets, respectively. Second row: ridge regression on \emph{bodyfat} and \emph{mg} datasets, respectively.}
% \label{fig:behaviour_of_tau}
% \end{center}
% \vspace{-0.75cm}
% \end{wrapfigure}

The theoretical analysis gives us the optimal   batch size for each of the proposed sampling techniques. However, we are unable to use these formulas directly since all of the expressions of optimal   batch size depend on the knowledge of $x^*$ through the values of $h_i^* \forall i \in [n]$. Our algorithm overcomes this problem by estimating the values of $h_i^*$ at every iteration by $h_i^k$. Although this approach seems to be mathematically sound, it is costly because it requires passing through the whole training set every iteration. Alternatively, a more practical approach is to store $h_i^0=h_i(x^0)\,\, \forall i \in [n]$, then set $h_i^k = \norm{\nabla f_i(x^k)}^2\,\, for\,\, i\in\mathcal S_k$ and $h_i^k = h_i^{k-1} \,\,for\,\, i \notin \mathcal S_k$, where $\mathcal S_k$ is the set of indices considered in the $k^{th}$ iteration. In addition to storing an extra $n$ dimensional vector, this approach costs only computing the norms of the stochastic gradients that we already used in the SGD step. Both options lead to convergence in a similar number of epochs, so we let our proposed algorithm adopt the second (more practical) option of estimating $h_i^*$.
% All three options lead to convergence in a similar number of epochs, so we let our proposed algorithm adopt the last (most practical) option of estimating $h_i^*$.

In our algorithm, for a given sampling technique, we use the current estimate of the model $x^k$ to estimate the sub-optimal   batch size $\tk := \tau(x^k)$ at the $k^{\text{th}}$ iteration. Based on this estimate, we use Lemmas \ref{le:L},\ref{le:variance} in calculating an estimate for both the expected smoothness  $\mathcal{L}(\tau^k)$ and the noise gradient $\sg(x^k, \tau^k)$ at that iteration. After that, we compute the step-size $\gamma^k$ using \eqref{eq:iteration_complexity} and finally conduct a SGD step \eqref{eq:SGD-MB}. The summary can be found in Algorithm \ref{alg:sgd_dyn_general}.

Note that intuitively, as $x^k$ gets closer to $x^*$, our estimate for the gradients at the optimum $h_i^k$ gets closer to $h_i^*$ and $\tk$ get closer to optimal   batch size $\tau(x^*)$. Later in this section, we show convergence of the iterates $x^0, x^1, \dots$ to a neighborhood of the solution $x^*$, and convergence of the sequence of batch estimates $\tau^1, \tau^2, \dots$ to a neighborhood around the optimal   batch size $\tau^*$.
% \begin{wrapfigure}{L}{0.5\textwidth}
%     \begin{minipage}{0.48\textwidth}
%         \begin{algorithm}
%             \caption{SGD with Dynamic   Batch size}
%             \label{alg:sgd_dyn_general}
%                 \begin{algorithmic}
%                     \STATE \textbf{Input:} Smoothness constants $L$, $L_i$, strong convexity constant $\mu$, target neighborhood $\epsilon$, Sampling Strategy $S$, initial point $x^0$, variance cap $C \geq 0$
%                     \STATE \textbf{Initialize:} Set $k=0$
%                     \WHILE{not converged}
%                         \STATE Set $\tau^k \leftarrow \tau(x^k)$ 
%                         \STATE Set $\lk \leftarrow \mathcal L(\tau^k)$
%                         \STATE Set $\sg^k \leftarrow \sg(x^k, \tau^k)$
%                         \STATE Set $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min(C,2\sg^k)} \right\}$ 
%                         \STATE Sample $v_k$ from $S$
%                         \STATE Do SGD step: $x^{k+1} \leftarrow x^k - \gamma^k \nabla f_{v_k} (x^k)$
%                         \STATE Update $k \leftarrow k+1$
%                     \ENDWHILE
%                     \STATE \textbf{Output:} $x^k$
%                 \end{algorithmic}
%         \end{algorithm}
%     \end{minipage}
% \end{wrapfigure}

% \begin{figure*}
% \begin{minipage}{width=0.5\textwidth}
% \centerline{
% \includegraphics[width=0.24\columnwidth]{figures/saga_experiments/mushrooms/Logistic_nice_Tau_mushrooms_1.png}
% \includegraphics[width=0.24\columnwidth,height=63.5pt]{figures/tau_evolution/logistic_nice_tau_a1a_1.png}
% }
% \centerline{
% \includegraphics[width=0.24\columnwidth]{figures/tau_evolution/ridge_nice_tau_bodyfat_1.png}
% \includegraphics[width=0.24\columnwidth]{figures/tau_evolution/ridge_ind_tau_mg_1.png}
% }
% \end{minipage}
% \begin{minipage}{width=0.5\textwidth}
% \centerline{
% \begin{algorithm}[t]
% \caption{SGD with Dynamic   Batch size}
% \label{alg:sgd_dyn_general}
% \begin{algorithmic}
% \STATE \textbf{Input:} Smoothness constants $L$, $L_i$, strong convexity constant $\mu$, target neighborhood $\epsilon$, Sampling Strategy $S$, initial point $x^0$, variance cap $C \geq 0$
% \STATE \textbf{Initialize:} Set $k=0$
% \WHILE{not converged}
%     \STATE Set $\tau^k \leftarrow \tau(x^k)$ 
%     \STATE Set $\lk \leftarrow \mathcal L(\tau^k)$
%     \STATE Set $\sg^k \leftarrow \sg(x^k, \tau^k)$
%     \STATE Set $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min(C,2\sg^k)} \right\}$ 
%     \STATE Sample $v_k$ from $S$
%     \STATE Do SGD step: $x^{k+1} \leftarrow x^k - \gamma^k \nabla f_{v_k} (x^k)$
%     \STATE Update $k \leftarrow k+1$
% \ENDWHILE
% \STATE \textbf{Output:} $x^k$
% \end{algorithmic}
% \end{algorithm}
% }
% \end{minipage}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure*}


% \begin{algorithm}[t]
% \caption{SGD with Adaptive   Batch size}
% \label{alg:sgd_dyn_general}
% \begin{algorithmic}
% \STATE \textbf{Input:} Smoothness constants $L$, $L_i$, strong convexity constant $\mu$, target neighborhood $\epsilon$, Sampling Strategy $S$, initial point $x^0$, variance cap $C \geq 0$
% \STATE \textbf{Initialize:} Set $k=0$
% \WHILE{not converged}
%     \STATE Set $\tau^k \leftarrow \tau(x^k)$ 
%     \STATE Set $\lk \leftarrow \mathcal L(\tau^k)$
%     \STATE Set $\sg^k \leftarrow \sg(x^k, \tau^k)$
%     \STATE Set $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min(C,2\sg^k)} \right\}$ 
%     \STATE Sample $v_k$ from $S$
%     \STATE Do SGD step: $x^{k+1} \leftarrow x^k - \gamma^k \nabla f_{v_k} (x^k)$
%     \STATE Update $k \leftarrow k+1$
% \ENDWHILE
% \STATE \textbf{Output:} $x^k$
% \end{algorithmic}
% \end{algorithm}

\begin{figure*}[t]
\begin{center}
\centerline{
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_nice_bodyfat_1.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_nice_bodyfat_2.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_nice_bodyfat_3.png}
\includegraphics[width=0.25\textwidth]{figures/Complexity/0Ridge_nice_bodyfat_1.png}
}
\centerline{
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_ind_mg_1.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_ind_mg_2.png}
\includegraphics[width=0.25\textwidth]{figures/saga_experiments/Ridge_ind_mg_3.png}
\includegraphics[width=0.25\textwidth]{figures/Complexity/0Ridge_nice_mg_1.png}
}
\caption{\textbf{Convergence of ridge regression} using $\tau-$partition nice sampling on \emph{bodyfat} dataset (first row) and $\tau-$partition independent sampling on \emph{mg} dataset (second row). In first three columns, training set is distributed among $1$, $2$ and $3$ partitions, respectively. Figures in the fourth column show how many epochs does the SGD need to converge for all   batch sizes (single partition dataset).
% On \emph{bodyfat} dataset, our algorithm outperforms SGD on $85.3\%$ of all possible fixed   batch sizes, while on \emph{mg} dataset, our algorithm outperforms SGD on $82.5\%$ of all fixed   batch sizes. In both cases, our algorithm can achieve a speedup of $300\%$.
}
\label{fig:ridge_nice}
\end{center}
\vspace{-0.75cm}
\end{figure*}

\textbf{Convergence of Algorithm \ref{alg:sgd_dyn_general}.}
Although the proposed algorithm is taking an SGD step at each iteration and we can derive one-step estimate (for $\gamma^k \leq \frac 1 {2 \mathcal L^k}$)
\begin{equation} \label{eq:one_step}
\Exp{\norm{x^{k+1}-x^*}^2 |x^k} \leq (1-\gamma^k \mu)\norm{x^k-x^*}^2 +2(\gamma^k)^2 \sg
,\end{equation}
the global behavior of our algorithm differs from SGD.
We dynamically update both the learning rate and the   batch size. At each iteration, we set the learning rate $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{2\sg^k} \right\}$, which depends on our estimates of both $\lk$ and $\sg^k$. If we were guaranteed that both of these terms are bounded above, then we can show that the sequence of generated learning rates will be lower bounded by a positive constant. In such cases, one can use inequality \eqref{eq:one_step} to prove the convergence of Algorithm \ref{alg:sgd_dyn_general}. To this end, we cap $\sg^k$ by a positive constant $C$, and we set the learning rate at each iteration to $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min\{C,2\sg^k\}} \right\}$. This way, we guarantee an upper bound of our estimate to the noise gradient at each iteration.
It is worth mentioning that this addition of the capping limit $C$ is for the theoretical treatment only and it is dropped in all of the conducted experiments. Now, we follow this informal description by rigorous formulations and we keep the proofs to the appendix.


\begin{lemma}\label{le:step_sizes_positive}
Learning rates generated by Algorithm \ref{alg:sgd_dyn_general} are bounded by positive constants $\gamma_{\max}= \tfrac 1 2\max_{\tau \in [n]} \left\{ \tfrac 1 {\mathcal L(\tau)} \right\}$ and $ \gamma_{\min}= \frac 1 2\min \left\{ \min_{\tau \in [n]} \left\{\tfrac 1 {\mathcal L(\tau)} \right\}, \tfrac{\epsilon \mu} C \right\} $.
\end{lemma}
We use Lemma \ref{le:step_sizes_positive} to bound $\gamma^k$ in Inequality \eqref{eq:one_step} to obtain the following convergence theorem. 
\begin{theorem}\label{th:convergence_our}
Assume $f$ is $\mu-$strongly convex and assumptions \ref{as:expected_smoothness}, and \ref{as:gradient_noise} hold. 
Then the iterates of Algorithm \ref{alg:sgd_dyn_general} satisfy:
\begin{equation} \label{eq:x_distance_bound}
\mathbb{E}\left\|x^k - x^*\right\|^2 \leq \left(1-\gamma_{\min}\mu\right)^k\left\|x^0-x^*\right\|^2 + R,
\end{equation} 
\end{theorem}


where $R = \tfrac{2\gamma_{\max}^2\sg^*}{\gamma_{\min}\mu}$. Note that the results above recover the earlier results of \cite{SGD_general_analysis} under fixed learning rate $\gamma^k = \gamma$. 
Theorem \ref{le:step_sizes_positive} guarantees the convergence of the proposed algorithm. Although there is no significant theoretical improvement here compared to previous SGD results in the fixed   batch and learning rate regimes, we measure the improvement to be significant in practice. 

\textbf{Convergence of $\tk$ to $\tau^*$}. The motivation behind the proposed algorithm is to learn the optimal   batch size in an online fashion so that we get to $\epsilon-$neighborhood of the optimal model with the minimum number of epochs. For simplicity, let's assume that $\sigma^*=0$. As $x^k \rightarrow x^*$, then $h_i^k=\nabla f_i(x^k) \rightarrow \nabla f_i(x^*) = h_i^*$, and thus  $\tk \rightarrow \tau^*$. 
In Theorem \ref{th:convergence_our}, we showed the convergence of $x^k$ to a neighborhood around $x^*$. Hence the theory predicts that our estimate of the optimal   batch $\tk$ will converge to a neighborhood of the optimal   batch size $\tau^*$ which was also confirmed by the experimental results in Figure \ref{fig:behaviour_of_tau}.





==> parts/papers/adaptive/sections/theoretical_analysis.tex <==
\section{Deriving Optimal   Batch Size} \label{sec:analysis}
After giving this thorough introduction to the stochastic reformulation of SGD, we can move on to study the effect of the   batch size on the total iteration complexity. In fact, for each sampling technique, the   batch size will affect both the expected smoothness $\mathcal{L}$ and the gradient noise $\sg$. This effect reflects on the number of iterations required to reach to $\epsilon$ neighborhood around the optimal model \eqref{eq:iteration_complexity}.

\textbf{Formulas for $\mathcal L$ and $\sigma$}
Before proceeding, we establish some terminologies. In addition of having $f$ to be $L-$smooth, we also assume each $f_i$ to be $L_i-$smooth.
In $\tau-$partition samplings (both nice and independent), let $n_{\mathcal C_j}$ be number of data-points in the partition $\mathcal C_j$, where $n_{\mathcal C_j} \geq \tau$. Let $L_{\mathcal C_j}$ be the smoothness constants of the function $f_{\mathcal C_j} = \tfrac{1}{n_{\mathcal C_j}}\sum_{i \in \mathcal C_j} f_i$. Also, let $\overline L_{\mathcal C_j} = \tfrac{1}{n_{\mathcal C_j}} \sum_{i\in\mathcal C_j} L_i$ be the average of the Lipschitz smoothness constants of the functions in partition $\mathcal C_j$. In addition, let $h_{\mathcal C_j}(x) = \norm{\nabla f_{\mathcal{C}_j}(x)}^2$ be the norm of the gradient of $f_{\mathcal{C}_j}$ at $x$. Finally, let $\overline {h}_{\mathcal C_j}(x) = \tfrac {1} {n_{\mathcal C_j}} \sum_{i \in C_j} h_i(x)$. For ease of notation, we will drop $x$ from all of the expression since it is understood from the context $(h_i = h_i(x))$. Also, superscripts with $(*,k)$ refer to evaluating the function at $x^*$ and $x^k$ respectively $(e.g.\,\, h_i^* = h_i(x^*))$.

Now we introduce our first key lemma, which gives an estimate of the expected smoothness for different sampling techniques, where the proof is left for the appendix.

\begin{lemma} \label{le:L}
For the considered samplings, the expected smoothness constants $\mathcal L$ can be upper bounded by $\mathcal L(\tau)$ (i.e. $\mathcal L \leq \mathcal L(\tau)$), where $\mathcal L(\tau)$ is expressed as follows.
(i) For $\tau$-partition nice sampling,
\begin{equation*} \label{eq:L_part_nice}
\mathcal L (\tau) = \tfrac{1}{n\tau} \max_{\mathcal C_j} \tfrac{n_{\mathcal C_j}}{q_{\mathcal C_j}(n_{\mathcal C_j}-1)} 
\Big[(\tau-1) L_{\mathcal C_j}n_{\mathcal C_j}
+ (n_{\mathcal C_j}-\tau) \max_{i \in{\mathcal C_j}}{L_i} \Big].
\end{equation*}

(ii) For $\tau$-partition independent sampling, $\mathcal L (\tau) = \tfrac{1}{n}\max_{\mathcal C_j}{\tfrac{n_{\mathcal C_j} L_{\mathcal C_j}}{q_{\mathcal C_j}} + \max_{i \in C_j}{\tfrac{L_i(1-p_{i})}{q_{C_j}p_{i}}}}.$
% \begin{equation*} 
% \mathcal L (\tau) = \tfrac{1}{n}\max_{\mathcal C_j}{\tfrac{n_{\mathcal C_j} L_{\mathcal C_j}}{q_{\mathcal C_j}} + \max_{i \in C_j}{\tfrac{L_i(1-p_{i})}{q_{C_j}p_{i}}}}.
% \end{equation*}
\end{lemma}

Note that (i), (ii) give as special case, for having all of the data in a single partition, the expected smoothness bound $\mathcal L(\tau)$ for $\tau$-nice sampling (without replacement) and $\tau$-independent sampling, which are results of \cite{SGD_general_analysis}. The bound on the expected smoothness constant for $\tau$-nice sampling without replacement is given by
$\mathcal L (\tau) = \tfrac {n(\tau-1)}{\tau(n-1)}L + \tfrac {n-\tau}{\tau(n-1)}\max_i L_{i},$
and that for $\tau$-independent sampling is given by
$\mathcal L (\tau) = L + \max_i \tfrac {1-p_i}{p_i}\tfrac {L_i} n.$


Next, we move to estimate the noise gradient $\sg (x^*, \tau)$ for different sampling techniques. The following lemma can accomplish this, where the proof is left for the appendix.

\begin{lemma} \label{le:variance}
For the considered samplings, the gradient noise is given by $\sg (x^*, \tau)$, where $\sg (x, \tau)$ is defined as:


(i) For $\tau$-partition nice sampling, $\sg(x,\tau) = \tfrac{1}{n^2\tau}\sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^2}{q_{\mathcal C_j}(n_{\mathcal C_j}-1)} \Big[(\tau-1)  h_{\mathcal C_j}n_{\mathcal C_j} 
 + (n_{\mathcal C_j}-\tau) \overline {h}_{\mathcal C_j}\Big].$
% \begin{align*} 
% \sg(x,\tau) = \tfrac{1}{n^2\tau}\sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^2}{q_{\mathcal C_j}(n_{\mathcal C_j}-1)} \Big[(\tau-1)  h_{\mathcal C_j}n_{\mathcal C_j} 
%  + (n_{\mathcal C_j}-\tau) \overline {h}_{\mathcal C_j}\Big]. 
% \end{align*}

(ii) For $\tau-$partition independent sampling, $\mathcal \sg(x,\tau) = \tfrac{1}{n^2}\sum_{\mathcal C_j}\tfrac{n_{\mathcal C_j}^2  h_{\mathcal C_j} + \sum_{i \in C_j}{\tfrac{1-p_{i}}{p_{i}} h_i}}{q_{C_j}}$

% \begin{equation*} \label{eq:sig_part_ind}
% \mathcal \sg(x,\tau) = \tfrac{1}{n^2}\sum_{\mathcal C_j}\tfrac{n_{\mathcal C_j}^2  h_{\mathcal C_j} + \sum_{i \in C_j}{\tfrac{1-p_{i}}{p_{i}} h_i}}{q_{C_j}}
% .\end{equation*}

\end{lemma}

Similarly, (i) and (ii) can be specialized in the case of having all of the data in a single partition to the gradient noise $\sg(x^*, \tau)$ for $\tau$-nice sampling (without replacement) and $\tau-$independent samplings, which are the results of \cite{SGD_general_analysis}. For $\tau-$nice sampling without replacement, we have
$\sg(x^*,\tau)=\tfrac {n-\tau} {n\tau(n-1)} \sum_{i \in [n]} h_i^*,$
and for $\tau-$independent sampling, we have
$\sg(x^*,\tau)=\tfrac 1 {n^2} \sum_{i \in [n]} \tfrac {1-p_i}{p_i}h_i^*.$

In what follows, we are going to deploy these two key lemmas to find expressions for the optimal   batch size that will minimize the total iteration complexity.




\textbf{Optimal   Batch Size}
Our goal is to estimate total iteration complexity as a function of $\tau$. In each iteration, we work with $\tau$ gradients, thus we can lower bound on the total iteration complexity by multiplying lower bound on iteration complexity \eqref{eq:iteration_complexity} by $\tau$.
We can apply similar analysis as in \cite{SGD_general_analysis}. 
Since we have estimates on both the expected smoothness constant and the gradient noise in terms of the   batch size $\tau$, we can lower bound total iteration complexity \eqref{eq:iteration_complexity} as
$$ T(\tau) = \tfrac 2 {\mu} \max \left\{ \tau\mathcal L(\tau), \tfrac{2}{\epsilon \mu}\tau \sg(x^*,\tau) \right\} \log\left( \tfrac{2 \|x^0 - x^*\|^2}{\epsilon} \right).$$
Note that if we are interested in minimizer of $T(\tau)$, we can drop all constant terms in $\tau$. Therefore, optimal   batch size $\tau^*$ minimizes $\max \left\{ \tau\mathcal L(\tau), \tfrac{2}{\epsilon \mu}\tau \sg(x^*,\tau) \right\}$. It turns out that all $\tau \mathcal L(\tau)$, and $\tau \sg(x^*,\tau)$ from Lemmas \ref{le:L}, \ref{le:variance} are piece-wise linear functions in $\tau$, which is cruicial in helping us find the optimal $\tau^*$ that minimizes $T(\tau)$.  Indeed, for the proposed sampling techniques, the optimal   batch size can be calculated from the following theorem, where its proof is left for the appendix.


\begin{theorem}\label{le:tau_star}
For $\tau$-partition nice sampling, the optimal   batch size is $\tau(x^*)$, where 
\begin{equation*} \label{eq:tau_part_nice}
 \tau(x) =    \min_{\mathcal C_r}\tfrac{
    \tfrac{nn_{\mathcal C_r}^2}{e_{\mathcal{C}_r}} (L_{\mathcal C_r}-L_{\max}^{\mathcal C_r}) + \tfrac{2}{\epsilon \mu} \sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^3}{e_{\mathcal C_j}}\left(\overline {h}_{\mathcal C_j}- h_{\mathcal C_j}\right)}
    {\tfrac {nn_{\mathcal{C}_r}} {e_{\mathcal C_r}}(n_{\mathcal C_r}L_{\mathcal C_r}-L_{\max}^{\mathcal{C}_r}) + \tfrac{2}{\epsilon \mu}\sum_{\mathcal C_j} 
    \tfrac{n_{\mathcal C_j}^2 }{e_{\mathcal C_j}}({\overline {h}_{\mathcal C_j} -n_{\mathcal C_j}  h_{\mathcal C_j} })}, \quad if  \quad\sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^2}{e_j} ( h_{\mathcal C_j}^*n_{\mathcal C_j}-\overline {h}^*_{\mathcal C_j}) \le 0,
\end{equation*}
% if  $\quad\sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^2}{e_j} ( h_{\mathcal C_j}^*n_{\mathcal C_j}-\overline {h}^*_{\mathcal C_j}) \le 0,$

where $e_{\mathcal C_k}=q_{\mathcal C_k} (n_{\mathcal C_k} -1)$, $L_{\max}^{\mathcal{C}_r}=\max_{i \in \mathcal C_r}{L_i}$. Otherwise: $\tau(x^*)=1$.

For $\tau-$partition independent sampling with $p_i = \frac{\tau}{n_{\mathcal C_j}}$, where $\mathcal C_j$ is the partition where i belongs, we get the optimal   batch size $\tau(x^*)$, where 

\begin{equation*} \label{eq:tau_part_ind}
    \tau(x) = \min_{\mathcal C_r}{\tfrac{
    \tfrac{2}{\epsilon \mu}
    \sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}^2} { q_{\mathcal C_j}} \overline {h}_{\mathcal C_j} - \tfrac{n}{q_{\mathcal C_r}} L_{\max}^{\mathcal{C}_r} }
    {
    \tfrac{2}{\epsilon \mu}\sum_{\mathcal C_j} \tfrac {n_{\mathcal C_j}} { q_{\mathcal C_j}}
    (\overline {h}_{\mathcal C_j} - n_{\mathcal C_j} h_{\mathcal C_j})
    +
    \tfrac n {q_{\mathcal C_r}} (n_{\mathcal C_r}L_{\mathcal C_r}-L_{\max}^{\mathcal C_r}) 
    }}, \quad if  \quad\sum_{\mathcal C_j} \tfrac{n_{\mathcal C_j}}
    { q_{\mathcal C_j}} (n_{\mathcal C_j}  h_{\mathcal C_j}^* - \overline {h}^*_{\mathcal C_j}) \le 0,
\end{equation*}
where $L_{\max}^{\mathcal C_r}=\max_{i \in \mathcal C_r}{L_i}$. Otherwise: $\tau(x^*)=1$.
\end{theorem} 


Moreover, if all of the data are stored in one partition, then \eqref{eq:tau_part_nice} becomes formulas for $\tau-$nice sampling and $\tau-$independent sampling which as an earlier result of \cite{SGD_general_analysis}.
% $\tau_{\text{nice}}(x^*) =n\tfrac{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}+L}{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}+nL} \, ,\, \tau_{\text{ind}}(x^*) =n\tfrac{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}}{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}+nL}.$
% and \eqref{eq:tau_part_ind} becomes formula for $\tau-$independent sampling from \cite{SGD_general_analysis}, 
% $$\tau(x^*) =n\tfrac{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}}{\tfrac 2 {\mu \epsilon}\overline h^* -L_{\max}+nL}.$$
Note that as $\epsilon \rightarrow 0$ then $\tau^* \rightarrow n$. It makes intuitive sense, for it means that if one aims to converge to actual minimizer, then SGD will turn to be gradient descent. On the other hand, as $\epsilon$ grows to be very large, optimal   batch shrinks to $1$. 
Also note that the larger the variance at the optimum, the larger the optimal   batch size is. If the variance at the optimum is negligible, as in the case in overparameterized models, then the optimal   batch size will be 1.



\begin{figure}[t]
\begin{minipage}{0.5\textwidth}
\begin{center}
\centerline{
\includegraphics[width=0.5\columnwidth]{figures/saga_experiments/mushrooms/Logistic_nice_Tau_mushrooms_1.png}
\includegraphics[width=0.5\columnwidth,height=63.5pt]{figures/tau_evolution/logistic_nice_tau_a1a_1.png}
}

\centerline{
\includegraphics[width=0.5\columnwidth]{figures/tau_evolution/ridge_nice_tau_bodyfat_1.png}
\includegraphics[width=0.5\columnwidth]{figures/tau_evolution/ridge_ind_tau_mg_1.png}
}
\caption{\textbf{Behavior of $\tau-$adaptive throughout training epochs.} First row: logistic regression on \emph{mushroom} and \emph{a1a} datasets, respectively. Second row: ridge regression on \emph{bodyfat} and \emph{mg} datasets, respectively.}
\label{fig:behaviour_of_tau}
\end{center}
\end{minipage}
\vspace{-0.7cm}
\begin{minipage}{0.5\textwidth}
\vspace{-0.6cm}
\begin{algorithm}[H]
\caption{SGD with Adaptive Batch size}
\label{alg:sgd_dyn_general}
\begin{algorithmic}
\STATE \textbf{Input:} Smoothness constants $L$, $L_i$, strong convexity constant $\mu$, target neighborhood $\epsilon$, Sampling Strategy $S$, variance cap $C \geq 0$, $x^0$
\STATE \textbf{Initialize:} Set $k=0$
\WHILE{not converged}
    \STATE Set $\tau^k \leftarrow \tau(x^k)$ 
    \STATE Set $\lk \leftarrow \mathcal L(\tau^k)$
    \STATE Set $\sg^k \leftarrow \sg(x^k, \tau^k)$
    \STATE Set $\gamma^k \leftarrow \frac 1 2 \min \left\{\frac 1 {\lk}, \frac{\epsilon \mu}{\min(C,2\sg^k)} \right\}$ 
    \STATE Sample $v_k$ from $S$
    \STATE Do SGD step: $x^{k+1} \leftarrow x^k - \gamma^k \nabla f_{v_k} (x^k)$
    \STATE Update $k \leftarrow k+1$
\ENDWHILE
\STATE \textbf{Output:} $x^k$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{figure}

==> parts/texts/Papers.tex <==

% Appendix for Papers

\refstepcounter{chapter}%
\chapter*{\thechapter \quad Papers Submitted and Under Preparation}

$\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, further attributes.\\
$\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, Mon. Year. \\
$\bullet$ Author 1 Name, Author 2 Name, and Author 3 Name, {``Article Title"}, \emph{Submitted to Conference/Journal Name}, Mon. Year.



==> parts/texts/comments.tex <==

% \begin{itemize}[leftmargin=*]
%     \item ML has long history. Modern world is data-driven, scale of data is huge, there is need for reliable and scalable ML. 
%     \item Optimization and discrepancy between theory algorithms and practical algorithms. Practical performance vs understanding.
%     \item Bridge divide is important, we tackle [list].
% \end{itemize}

% Namely, we investigate following aspects of the training process:
% \begin{itemize}
% \item loss-function choice
% \item post-training fine-tuning, perso
% \item unknown hyperparameters
% \item model initialization far from the solution
% \item cheap versions of Hessian oracle 
% \end{itemize}

% \begin{itemize}[leftmargin=*]
%     \item Why did we achieved.
% \end{itemize}

% \subsection*{Motivation draft:}

% Machine Learning has long history. Modern world is data-driven, scale of data is huge, there is need for reliable and scalable ML. 

% We focus on the Optimization part, how to train Machine Learning models fast and reliably. There is a large discrepancy between well-understood algorithms and heuristics used in practice.

% Popular algorithms lack theoretical guarantees, but coupled with ad-hoc engineering tricks performs surprisingly well.
% On the real-world tasks, they out-compete theoretically-based algorithms by a substantial margin.
% However, they are often black box and not interpretable. Their understanding relies heavily on empirical performance.

% We leverage already developed theory and observations from practice in order to bridge this divide.

% We strive to develop more reliable, interpretable, and scalable machine learning models that can confidently drive modern data-driven applications.



% $\bullet$ Q: What is the price of the FL personalization if we fix personalization pre-training?\\
% $\bullet$ paper: Optimal algorithms for personalized FL\\
% $\bullet$ A: as expensive as centralized training\\

% \noindent
% $\bullet$ Q: If we personalize by post-training fine-tuning, what convergence can we guarantee?\\
% $\bullet$ paper: \fomaml{}\\
% $\bullet$ A: popular \fomaml{} has \sgd{} rate do different objective\\

% \noindent
% $\bullet$ Q: Optimal minibatch size formula [Gower] is purely theoretical. Is it of any use?\\
% $\bullet$ paper: Adaptive learning of minibatch size\\
% $\bullet$ A: Yes. We present a approximation heuristic with convergence guarantees\\

% % \subsubsection*{Beyond first-order methods:}

% \noindent
% $\bullet$ Q: Newton-like methods converge extremely quickly, but they depend on initialization. Are there simple and fast globally convergent methods?\\
% $\bullet$ paper: AICN\\
% $\bullet$ A: yes, AICN\\

% \noindent
% $\bullet$ Q: Can Newton-like methods have cheap iteartions and fast convergence in the same time?\\
% $\bullet$ paper: SGN\\
% $\bullet$ A: yes, SGN\\


% Machine Learning (ML) has an extensive history and has become increasingly pivotal in our data-driven world. The scale of available data has grown exponentially, necessitating the development of reliable and scalable ML methods. This dissertation focuses on the optimization aspect of ML, specifically addressing the need for fast and dependable training of ML models. However, a significant disparity exists between well-understood algorithms and the heuristics employed in practice.
